Chart Question Answering: State of the Art and Future Directions

Information visualizations such as bar charts and line charts are very common for analyzing data and discovering critical insights. Often people analyze charts to answer questions that they have in mind. Answering such questions can be challenging as they often require a significant amount of perceptual and cognitive effort. Chart Question Answering (CQA) systems typically take a chart and a natural language question as input and automatically generate the answer to facilitate visual data analysis. Over the last few years, there has been a growing body of literature on the task of CQA. In this survey, we systematically review the current state-of-the-art research focusing on the problem of chart question answering. We provide a taxonomy by identifying several important dimensions of the problem domain including possible inputs and outputs of the task and discuss the advantages and limitations of proposed solutions. We then summarize various evaluation techniques used in the surveyed papers. Finally, we outline the open challenges and future research opportunities related to chart question answering.

==> biography.tex <==
\newpage

\noindent \textbf{Short Biographies of Authors}

\noindent \textbf{Enamul Hoque} 

\noindent Enamul Hoque is an Assistant Professor 
%in the School of Information Technology 
at York University where he directs the Intelligent Visualization Lab. Previously, he was a postdoctoral fellow 
%Computer Science
at Stanford University. He received the Ph.D. degree in Computer Science from the University of British Columbia. His research focuses on combining information visualization and human-computer interaction with natural language processing to address the challenges of the information overload problem.  
%In recent work, he focuses on how to perform natural language interactions with information visualization. 
Along with his collaborators he developed several  natural language interfaces for supporting data analyis and question answering with visualizations~\cite{hoque2017applying, sneak-peak, miva-2021}. He has also worked on question answering with charts \cite{Kim2020, ahmed-workshop-2021} as well as generating visual explanations \cite{Kim2020} and summaries from  charts~\cite{obeid-inlg}.  
%His research addresses the challenges of the information overload problem using an interdisciplinary lens, combining information visualization and human-computer interaction with natural language processing.
His research has been supported by Natural Sciences and Engineering Research Council of Canada, National Research Council Canada, and Canada Foundation for Innovation among others. 

\noindent \textbf{Parsa Kavehzadeh}

\noindent Parsa Kavehzadeh is a graduate student in Computer Science at York University where he works with Enamul Hoque. He completed his BSc from Amirkabir University of Tech. His research interests includes information visualization, question answering, natural language generation, and deep learning. Currently, he is working on developing machine learning techniques for supprting conversational question answering with charts.


\noindent \textbf{Ahmed Masry}

\noindent Ahmed Masry is pursuing MSc in Computer Science degree at York University under the supervision of Enamul Hoque. He completed his BSc from Koc University in Turkey. His research interests includes chart question answer, deep learning, computer vision, and natural language processing. In particular, he focuses on answering factual question about charts~\cite{ahmed-workshop-2021}.
